Accelerating MRI with Longitudinally-informed Latent Posterior Sampling

Purpose: To accelerate MRI acquisition by incorporating the previous scans of a subject during reconstruction. Although longitudinal imaging constitutes much of clinical MRI, leveraging previous scans is challenging due to the complex relationship between scan sessions, potentially involving substantial anatomical or pathological changes, and the lack of open-access datasets with both longitudinal pairs and raw k-space needed for training deep learning-based reconstruction models. Methods: We propose a diffusion-model-based reconstruction framework that eliminates the need for longitudinally paired training data. During training, we treat all scan timepoints as samples from the same distribution, therefore requiring only standalone images. At inference, our framework integrates a subject's prior scan in magnitude DICOM format, which is readily available in clinical workflows, to guide reconstruction of the follow-up. To support future development, we introduce an open-access clinical dataset containing multi-session pairs including prior DICOMs and follow-up k-space. Results: Our method consistently outperforms both longitudinal and non-longitudinal baseline reconstruction methods across various accelerated Cartesian acquisition strategies. In imaging regions highly similar to the prior scan, we observe up to 10\% higher SSIM and 2 dB higher PSNR, without degradation in dissimilar areas. Compared to longitudinal reconstruction baselines, our method demonstrates robustness to varying degrees of anatomical change and misregistration. Conclusion: We demonstrate that prior scans can be effectively integrated with state-of-the-art diffusion-based reconstruction methods to improve image quality and enable greater scan acceleration, without requiring an extensive longitudinally-paired training dataset.

==> shortcuts.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would not end up as ``with respect toblah''. 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

% includes
\usepackage{amsmath, amssymb} 
\usepackage{amsmath}
\usepackage{bm}
\usepackage{xcolor}

\DeclareMathOperator{\Tr}{Tr}

\newcommand{\footnotestandalone}[1]{\let\thefootnote\relax\footnotetext{#1}}
\newcommand{\indicator}[1]{\mathbf{1}_{\{#1\}}}

% Numbers
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}

% colors
\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\bRED}[1]{{{\textbf{\RED{#1}}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}  
\newcommand{\bBLUE}[1]{{{\textbf{\BLUE{#1}}}}}  

\newcommand{\TBD}{\RED{[TBD]}}

\newcommand{\TODO}[1]{\RED{[TODO: #1]}}

% % Command abbreviations
\newcommand{\beite}{\begin{itemize}}
\newcommand{\enite}{\end{itemize}}
\newcommand{\beenu}{\begin{enumerate}}
\newcommand{\enenu}{\end{enumerate}}
\newcommand{\becen}{\begin{center}}
\newcommand{\encen}{\end{center}}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% \newcommand{\prox}{\text{prox}}
\newcommand{\prox}{{\mathrm{prox}}}
\newcommand{\minop}[1]{\ensuremath{\operatorname*{min}_{#1}}}
\newcommand{\maxop}[1]{\ensuremath{\operatorname*{max}_{#1}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}
\newcommand{\arginf}[1]{\ensuremath{\operatorname*{arg\,inf}_{#1}}}
\newcommand{\argsup}[1]{\ensuremath{\operatorname*{arg\,sup}_{#1}}}


\makeatletter
\newcommand*{\indep}{%
  \mathbin{%
    \mathpalette{\@indep}{}%
  }%
}
\newcommand*{\nindep}{%
  \mathbin{%                   % The final symbol is a binary math operator
    \mathpalette{\@indep}{\not}% \mathpalette helps for the adaptation
                               % of the symbol to the different math styles.
  }%
}
\newcommand*{\@indep}[2]{%
  % #1: math style
  % #2: empty or \not
  \sbox0{$#1\perp\m@th$}%        box 0 contains \perp symbol
  \sbox2{$#1=$}%                 box 2 for the height of =
  \sbox4{$#1\vcenter{}$}%        box 4 for the height of the math axis
  \rlap{\copy0}%                 first \perp
  \dimen@=\dimexpr\ht2-\ht4-.2pt\relax
      % The equals symbol is centered around the math axis.
      % The following equations are used to calculate the
      % right shift of the second \perp:
      % [1] ht(equals) - ht(math_axis) = line_width + 0.5 gap
      % [2] right_shift(second_perp) = line_width + gap
      % The line width is approximated by the default line width of 0.4pt
  \kern\dimen@
  {#2}%
      % {\not} in case of \nindep;
      % the braces convert the relational symbol \not to an ordinary
      % math object without additional horizontal spacing.
  \kern\dimen@
  \copy0 %                       second \perp
} 
\makeatother

\newcommand*{\nperp}{\not\perp}

% expectation
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}\mathrm{ar}}

% bolds
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bd}{{\bf d}}
\newcommand{\be}{{\bf e}}
\newcommand{\bdf}{{\bf f}}
\newcommand{\bg}{{\bf g}}
\newcommand{\bh}{{\bf h}}
\newcommand{\bi}{{\bf i}}
\newcommand{\bj}{{\bf j}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bl}{{\bf l}}
% \newcommand{\bm}{{\bf m}}
\newcommand{\bn}{{\bf n}}
\newcommand{\bo}{{\bf o}}
\newcommand{\bp}{{\bf p}}
\newcommand{\bq}{{\bf q}}
\newcommand{\br}{{\bf r}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bt}{{\bf t}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bz}{{\bf z}}
\newcommand{\beps}{{\boldsymbol{\epsilon}}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bG}{{\bf G}}
\newcommand{\bH}{{\bf H}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bJ}{{\bf J}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bL}{{\bf L}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bO}{{\bf O}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bQ}{{\bf Q}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bW}{{\bf W}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bZ}{{\bf Z}}

% bold greek
\newcommand{\balpha}{{\bm{\alpha}}}
\newcommand{\bbeta}{{\bm{\beta}}}
\newcommand{\bgamma}{{\bm{\gamma}}}
\newcommand{\bdelta}{{\bm{\delta}}}
\newcommand{\bepsilon}{{\bm{\epsilon}}}
\newcommand{\bzeta}{{\bm{\zeta}}}
\newcommand{\btheta}{{\bm{\theta}}}
\newcommand{\biota}{{\bm{\iota}}}
\newcommand{\bkappa}{{\bm{\kappa}}}
\newcommand{\blambda}{{\bm{\lambda}}}
\newcommand{\bmu}{{\bm{\mu}}}
\newcommand{\bnu}{{\bm{\nu}}}
\newcommand{\bxi}{{\bm{\xi}}}
\newcommand{\bomicron}{{\bm{\omicron}}}
\newcommand{\bpi}{{\bm{\pi}}}
\newcommand{\brho}{{\bm{\rho}}}
\newcommand{\bsigma}{{\bm{\sigma}}}
\newcommand{\btau}{{\bm{\tau}}}
\newcommand{\bupsilon}{{\bm{\upsilon}}}
\newcommand{\bphi}{{\bm{\phi}}}
\newcommand{\bchi}{{\bm{\chi}}}
\newcommand{\bpsi}{{\bm{\psi}}}
\newcommand{\bomega}{{\bm{\omega}}}

\newcommand{\bGamma}{{\bm{\Gamma}}}
\newcommand{\bDelta}{{\bm{\Delta}}}
\newcommand{\bTheta}{{\bm{\Theta}}}
\newcommand{\bLambda}{{\bm{\Lambda}}}
\newcommand{\bXi}{{\bm{\Xi}}}
\newcommand{\bPi}{{\bm{\Pi}}}
\newcommand{\bSigma}{{\bm{\Sigma}}}
\newcommand{\bUpsilon}{{\bm{\Upsilon}}}
\newcommand{\bPhi}{{\bm{\Phi}}}
\newcommand{\bPsi}{{\bm{\Psi}}}
\newcommand{\bOmega}{{\bm{\Omega}}}

% calligraphy
\newcommand{\cA}{{\cal A}}
\newcommand{\bcA}{{\bf \cal A}}
\newcommand{\bcP}{{\bf \cal P}}
\newcommand{\bcD}{{\bf \cal D}}
\newcommand{\bcE}{{\bf \cal E}}
\newcommand{\bcF}{{\bf \cal F}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}

\newcommand{\bone}{{\bf 1}}
\newcommand{\bzr}{{\bf 0}}


% Norm
\newcommand{\ellOne}{\ensuremath{{\ell_1}}}
\newcommand{\ellTwo}{\ensuremath{{\ell_2}}}
\newcommand{\ellp}{\ensuremath{{\ell_p}}}
\newcommand{\ellInfty}{\ensuremath{{\ell_\infty}}}

% It is better not to use ensuremath for these norms, as they would look funny when, e.g., they are squared.
\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\ellOneNorm}[1]{{\norm{#1}_{\ellOne}}}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellpNorm}[1]{{\norm{#1}_{\ellp}}}
\newcommand{\ellInftyNorm}[1]{{\norm{#1}_{\ellInfty}}}
\newcommand{\Fnorm}[1]{\left\|{#1}\right\|_F}

\newcommand{\ellTwoDist}[2]{d(#1,#2)_\ellTwo}
\newcommand{\ellOneDist}[2]{d(#1,#2)_\ellOne}
\newcommand{\SigmaDist}[2]{d(#1,#2)_\Sigma}

\newcommand{\Fdist}[2]{{d(#1,#2)_F}}

\newcommand{\DistExt}[2]{{d(#1,#2)_{\mathrm{Ext}}}}

\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\SOthree}{\mathrm{SO}(3)}
\newcommand{\sothree}{\mathfrak{so}(3)}

\newcommand{\SE}[1]{\ensuremath{\mathrm{SE(#1)}}}
\newcommand{\se}[1]{\ensuremath{\mathrm{se(#1)}}}

\newcommand{\GL}[1]{\ensuremath{\mathrm{GL(#1)}}}
\newcommand{\gl}[1]{\ensuremath{\mathrm{gl(#1)}}}
\newcommand{\GLn}{\GL{n}}
\newcommand{\GLthree}{\GL{3}}

\newcommand{\tp}{t_p}
\newcommand{\nopt}{n_{\rm{opt}}}

\newcommand{\GLnPlus}{\ensuremath{\mathrm{GL_{+}(n)}}}

\newcommand{\gln}{\ensuremath{\mathfrak{gl}(n)}}


\newcommand{\FRAME}[2]{
\begin{frame}
\begin{frametitle}{#1}
\end{frametitle}
#2
\end{frame}}

\newcommand{\BLOCK}[2]{
\begin{block}{#1}
#2
\end{block}}

\newcommand{\Ncols}{{N_{\text{cols}}}}
\newcommand{\Nrows}{{N_{\text{rows}}}}

\newcommand{\Nedges}{{N_{\text{edges}}}}


\newcommand\comment[1]{\textcolor{red}{#1}}

% dataset
\newcommand{\Dataset}{\mathfrak{D}}
\newcommand{\Validation}{\mathfrak{D}_v}

% fig captioning
\usepackage[justification=centering]{caption}
\usepackage{subcaption}

\newcommand{\DiffusionStep}{\operatorname{Diffusion-Step}}
\newcommand{\DDIMStep}{\operatorname{DDIM-Step}}
\newcommand{\CG}{\operatorname{CG-SENSE}}
\newcommand{\xinit}{\bx_{\rm{init}}}
\newcommand{\zinit}{\bz_{\rm{init}}}
\newcommand{\xside}{\bx_s}
\newcommand{\xgt}{\bx^\star}
\newcommand{\zgt}{\bz^\star}
\newcommand{\balph}{\bar{\alpha}_t}
\newcommand{\xp}{\bx^{\text{P}}}
\newcommand{\zp}{\bz^{\rm{P}}}


\newcommand{\abart}{\bar \alpha_t}
\newcommand{\tpemp}{t_p^{\star, \rm{obs}}}
\newcommand{\tpapprox}{{\tilde t}_{p}}

\newcommand{\tpscale}{v_{\rm{p}}}
\newcommand{\tpshift}{w_{\rm{p}}}

\newcommand{\tprev}{t_{\rm{prev}}}
\newcommand{\zprev}{\bz_{\rm{prev}}}
\newcommand{\tstep}{\Delta t}
\newcommand{\nstep}{n_{\rm{step}}}
\newcommand{\navg}{n_{\rm{avg}}}
\newcommand{\mineq}{-=}

\newcommand\bitsmall{\fontsize{9}{11}\selectfont}

\newcommand{\myoperatorname}[1]{\mathop{\texttt{#1}}\nolimits}
